Rethinking the Producer-Consumer Relationship in Modern DRAM-Based Systems

Generational improvements to commodity DRAM throughout half a century have long solidified its prevalence as main memory across the computing industry. However, overcoming today's DRAM technology scaling challenges requires new solutions driven by both DRAM producers and consumers. In this paper, we observe that the separation of concerns between producers and consumers specified by industry-wide DRAM standards is becoming a liability to progress in addressing scaling-related concerns. To understand the problem, we study four key directions for overcoming DRAM scaling challenges using system-memory cooperation: (i) improving memory access latencies; (ii) reducing DRAM refresh overheads; (iii) securely defending against the RowHammer vulnerability; and (iv) addressing worsening memory errors. We find that the single most important barrier to advancement in all four cases is the consumer's lack of insight into DRAM reliability. Based on an analysis of DRAM reliability testing, we recommend revising the separation of concerns to incorporate limited information transparency between producers and consumers. Finally, we propose adopting this revision in a two-step plan, starting with immediate information release through crowdsourcing and publication and culminating in widespread modifications to DRAM standards.

==> sections/authors.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{submission_goodies/photo_minesh.jpg}}]{Minesh Patel}
    received his Ph.D. from ETH Zürich and dual B.S. degrees from UT
    Austin in physics and electrical engineering. His doctoral thesis focuses on
    overcoming performance, reliability, and security challenges in the memory
    system. In particular, his dissertation identifies and addresses new challenges
    for system-level error detection and mitigation targeting memory chips with
    integrated error correcting codes (ECC). He also worked collaboratively on
    understanding and solving the RowHammer vulnerability,  near-data processing,
    efficient virtual memory management, and new hardware security primitives.
    Minesh's graduate work has been recognized with several honors, including DSN'19
    and MICRO’20 Best Paper Awards, the William Carter Dissertation Award in
    Dependability, the ETH Doctoral Medal, and induction into the ISCA Hall of Fame. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{submission_goodies/photo_taha_michael.jpg}}]{Taha Shahroodi}
    is a scientific researcher in two research groups:
    (1) the Quantum \& Computer Engineering department at Technische Universiteit
    Delft (TU Delft) and SAFARI Research Group at Technische Hochschule Zürich
    (ETH Zürich). Previously, Taha received a B.Sc. degree in computer
    engineering from the Sharif University of Technology (SUT) in 2018 and an
    M.Sc. degree in computer science from ETH Zürich in 2020. He worked on
    Machine Learning and Genomics system development for years and is currently
    investigating how to combine system analysis, machine learning, and genomics
    with modern storage and memory devices.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{submission_goodies/photo_aditya.jpg}}]{Aditya Manglik}
    earned a Master's in Electrical Engineering from ETH Zürich, Switzerland in
    2024 and a Bachelor's in Electrical Engineering from BITS Pilani in 2018. He
    is a graduate student advised by Prof. Onur Mutlu at the SAFARI Research
    Group, ETH Zürich. His research interests include sustainable systems,
    energy-efficient systems, secure system design, and Processing-in-Memory.
    For more information, please see his webpage at
    https://adityamanglik.github.io/.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{submission_goodies/photo_giray.jpg}}]{Abdullah Giray Ya{\u{g}}l{\i}k{\c{c}}{\i}}
    is a Ph.D. candidate in the Safari Research Group at
    ETH Zürich, working with Prof. Onur Mutlu. His current broader research
    interests are computer architecture, systems, and hardware security,
    focusing on DRAM robustness and performance. In particular, his Ph.D.
    research focuses on understanding and solving the RowHammer vulnerability,
    on which he has several publications. Giray received his B.S. degree in
    Electrical Engineering and M.Sc. degree in Computer Engineering from TOBB
    University of Economics and Technology, Ankara, Turkiye and he holds a
    second M.Sc. in Computer Science from University of Notre Dame, IN, USA.
    Giray holds an honorable mention from the Intel Hardware Security Academic
    Award, 2021, and is the First-Place winner in the graduate category of
    Student Research Competition in PACT, 2023. Giray's research is partly
    supported by Google and the Microsoft Swiss Joint Research Center. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{submission_goodies/photo_ataberk.png}}]{Ataberk Olgun}
    is a Ph.D. student at ETH Zürich. He received his master's
    degree in Computer Engineering from TOBB University of Economics and
    Technology. His research interests include memory system reliability,
    safety, and performance. For more information, please see his webpage at
    https://aolgun.com.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{submission_goodies/photo_richard.jpg}}]{Haocong Luo}
    is a Ph.D. student in the Safari Research Group at ETH Zürich,
    advised by Prof. Onur Mutlu. His current research interests are in computer
    architecture, focusing on memory systems and DRAM. Haocong received his B.
    Eng. degree in Computer Science from ShanghaiTech University, and his M.Sc.
    degree in Computer Science from ETH Zurich.

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{submission_goodies/photo_onur.jpg}}]{Onur Mutlu}
    (Fellow, IEEE) received the B.S. degree in computer engineering
    and psychology from the University of Michigan, Ann Arbor, and the M.S. and
    Ph.D. degrees in electrical and computer engineering from The University of
    Texas at Austin. He started the Computer Architecture Group, Microsoft
    Research (2006-2009) and has held various product and research positions
    with Intel Corporation, Advanced Micro Devices, VMware, and Google. He is
    currently a Professor of computer science with ETH Zürich. He is also a
    Faculty Member with Carnegie Mellon University, where he previously held the
    Strecker Early Career Professorship. A variety of techniques that he, along
    with his group and collaborators, has invented over the years have
    influenced the industry and have been employed in commercial microprocessors
    and memory/storage systems. His research interests include computer
    architecture, systems, hardware security, and bioinformatics. He is an ACM
    Fellow and an elected member of the Academy of Europe (Academia Europaea).
    He received the IEEE High-Performance Computer Architecture Test of Time
    Award, the IEEE Computer Society Edward J. McCluskey Technical Achievement
    Award, the ACM SIGARCH Maurice Wilkes Award, the inaugural IEEE Computer
    Society Young Computer Architect Award, the inaugural Intel Early Career
    Faculty Award, the U.S. National Science Foundation CAREER Award, the
    Carnegie Mellon University Ladd Research Award, the faculty partnership
    awards from various companies, and a healthy number of best paper or “top
    pick” paper recognitions at various computer systems, architecture, and
    security venues. His computer architecture and digital logic design course
    lectures and materials are freely available on YouTube
    (https://www.youtube.com/OnurMutluLectures), and his research group makes a
    wide variety of software and hardware artifacts freely available online
    (https://safari.ethz.ch/). For more information, please see his webpage at
    https://people.inf.ethz.ch/omutlu/.
\end{IEEEbiography}

